Design and analysis of a microplate assay in the presence of multiple restrictions on the randomization

Experiments using multi-step protocols often involve several restrictions on the randomization. For a specific application to in vitro testing on microplates, a design was required with both a split-plot and a strip-plot structure. On top of two-level treatment factors and the factors that define the randomization restrictions, a multi-level fixed blocking factor not involving further restrictions on the randomization had to be added. We develop a step-by-step approach to construct a design for the microplate experiment and analyze a response. To consolidate the approach, we study various alternative scenarios for the experiment.

==> figures/structure_diagram_scenario_1.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}[4]{*}{Week}    & \multirow{2}[4]{*}{Plate} & \multicolumn{16}{c|}{Tube} \\
    \cline{3-18}                &                           & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\
    \hline
    \multirow{2}[4]{*}{1}       & 1                         & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ &  & & & &   &   &   &   &   &   &   &  \\
    \cline{2-18}                & 2                         &  & & & & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ &   &   &   &   &   &   &   &  \\
    \hline
    \multirow{2}[4]{*}{2}       & 3                         &   &   &   &   &   &   &   &   & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ & & & & \\
    \cline{2-18}                & 4                         &   &   &   &   &   &   &   &   & & & & & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ & $\bullet \bullet$ \\
    \hline
\end{tabular}
